Benign Shortcut for Debiasing: Fair Visual Recognition via Intervention with Shortcut Features

Machine learning models often learn to make predictions that rely on sensitive social attributes like gender and race, which poses significant fairness risks, especially in societal applications, such as hiring, banking, and criminal justice. Existing work tackles this issue by minimizing the employed information about social attributes in models for debiasing. However, the high correlation between target task and these social attributes makes learning on the target task incompatible with debiasing. Given that model bias arises due to the learning of bias features (\emph{i.e}., gender) that help target task optimization, we explore the following research question: \emph{Can we leverage shortcut features to replace the role of bias feature in target task optimization for debiasing?} To this end, we propose \emph{Shortcut Debiasing}, to first transfer the target task's learning of bias attributes from bias features to shortcut features, and then employ causal intervention to eliminate shortcut features during inference. The key idea of \emph{Shortcut Debiasing} is to design controllable shortcut features to on one hand replace bias features in contributing to the target task during the training stage, and on the other hand be easily removed by intervention during the inference stage. This guarantees the learning of the target task does not hinder the elimination of bias features. We apply \emph{Shortcut Debiasing} to several benchmark datasets, and achieve significant improvements over the state-of-the-art debiasing methods in both accuracy and fairness.

==> tables/debiasing.tex <==
\begin{table}[t] 
  \caption{Social bias(in $\%$) in VLP models with different debiasing pre-training tasks. }
  \label{debias_result}
  	\resizebox{0.46\textwidth}{!}
{
	\begin{tabular}	{l   |  c  c  c | c  c  c  }
		\toprule	 	
	 \multirow{2}{*}{Method} & \multicolumn{3}{c|}{Activity 13K} &\multicolumn{3}{c}{Occupation 11K}\\
	 	 &B@V-L &B@V&B@L& B@V-L &B@V&B@L \\
    \midrule
    	vanilla  & 13.02 &11.10&4.89&14.84& 14.23 &3.15 \\
    	GS & 11.21 &9.25&4.03&12.47& 12.35 &2.98 \\
    	DR & 11.17 &9.54&4.39&13.52& 12.19 &3.08 \\
    	CycleGAN & 10.92 &9.23&4.32&12.07& 11.35 &3.01 \\

    	    \midrule
    	
    	FairVLP-V  & 8.41 &7.23&3.91&9.11& 7.98 &2.86 \\
    	FairVLP-L  & 8.53 &7.46&3.82&11.23& 9.61 &1.77 \\
    	    \midrule
    	FairVLP  & \textbf{6.97} &\textbf{6.76}&\textbf{3.29}&\textbf{7.74}& \textbf{7.15} &\textbf{1.72} \\

  \bottomrule
\end{tabular}
}
\end{table}


==> tables/main_result1.tex <==
\begin{table}[t]
  \caption{The social bias (in $\%$) in VLP models in terms of multi-modal bias(B@V-L), visual modal bias(B@V), and language modal bias(B@L). 
  For each bias, we used four text templates to measure bias and calculate the average(Avg.).}
  
%   For each bias, we used four text templates to measure bias and calculate the aug.For each bias, we calculated using four text templates: Sentence w/o specify(S$_\text{W/O}$), Sentence w/ specify(S$_\text{W/}$), Phrase w/o specify(P$_\text{W/O}$) and Phrase w/ specify(P$_\text{W/}$)
  
%     \small
% 	\centering	
%     \aboverulesep = 0.46mm
%     \belowrulesep = 0.46mm
% \setlength\tabcolsep{5pt}
	\resizebox{0.48\textwidth}{!}
{
	\begin{tabular}	{l  l |  c  c  c | c  c  c  }
		\toprule
% 		\multirow{2}{*}{\multirow{2}{*}{VLPs}}
	 & & \multicolumn{3}{c|}{Activity 13K} &\multicolumn{3}{c}{Occupation 11K}\\

	 
% 	  &  \multicolumn{3}{c}{TR}& \multicolumn{3}{c}{IR} \\
% 	 \midrule
	 &&B@V-L &B@V&B@L& B@V-L &B@V&B@L \\
    \midrule
	

	\multirow{5}{*}{\rotatebox{90}{ALBEF}}  &S$_\text{W/O}$& 10.29 &9.44&3.98& 13.31 &9.62&2.38 \\
	 &S$_\text{W/}$& 11.33 &6.54&7.15& 16.00 &10.46&6.46 \\&P$_\text{W/O}$ & 10.75 &8.21&4.27& 11.85 &7.85&1.69 \\ &P$_\text{W/}$ & 9.85 &7.54&3.31& 11.31 &8.23&2.08 \\ &Avg.& \textbf{10.56} &\textbf{7.93}&\textbf{4.68}& \textbf{13.12} &\textbf{9.04}&\textbf{3.15} \\
	     \midrule
	\multirow{5}{*}{\rotatebox{90}{TCL}}  &S$_\text{W/O}$& 7.62&6.96&3.67& 12.00 &10.85&3.92 \\
	&S$_\text{W/}$ & 8.94 &6.15&5.50& 16.46 &12.01&6.00 \\ &P$_\text{W/O}$& 7.52 &5.90&2.65& 10.15 &6.85&4.77 \\ &P$_\text{W/}$ & 6.88 &5.38&2.37& 8.38 &5.46&2.85 \\&Avg. & \textbf{7.74} &\textbf{6.10}&\textbf{3.55}& \textbf{11.75} &\textbf{8.79}&\textbf{4.84} \\
	     \midrule

	\multirow{5}{*}{\rotatebox{90}{ViLT}} &S$_\text{W/O}$ & 8.62 &6.52&2.37&16.15& 17.23 &3.62 \\
	 &S$_\text{W/}$&9.48& 8.71 &2.35&14.92& 17.35 &4.62 \\& P$_\text{W/O}$&14.65& 14.38 &2.27&12.92& 17.61 &3.38 \\ &P$_\text{W/}$ & 11.19 &11.85&1.69& 13.23 &15.15&4.46 \\ &Avg.& \textbf{10.99} &\textbf{10.37}&\textbf{2.17}& \textbf{14.31} &\textbf{16.84}&\textbf{4.02} \\

		\bottomrule
	\end{tabular}
 	}
%  	 \vspace{-0.8ex}
% 	\caption
% 	{
% % 	\small	
% 		
% 	}
	\label{main_result}
    % \vspace{-0.7ex}
\end{table}		



==> tables/main_result2.tex <==
\begin{table}[t]

  \caption{The social bias in language modality of three VLP models and language model BERT.}
  	\label{vlps-bert}
  
%     \small
% 	\centering	
%     \aboverulesep = 0.46mm
%     \belowrulesep = 0.46mm
% \setlength\tabcolsep{5pt}
% 	\resizebox{0.75\textwidth}{!}
{
	\begin{tabular}	{l   |  c  c  c  c   }
		\toprule	 	
	 \multirow{1}{*}{Target concept} &  ALBEF &TCL&ViLT& BERT \\

	\midrule
	52 Activities & 0.53 & 0.59 & 0.39 & \textbf{0.15}\\
	13 Occupations  & 0.69 & 0.71 & 0.48 &\textbf{0.20}\\
		\bottomrule
	\end{tabular}
%  	}
%  	 \vspace{-0.8ex}
% 	\caption
% 	{
% % 	\small	
% 		
% 	}
}
    % \vspace{-0.7ex}
\end{table}		

==> tables/retrieval.tex <==
\begin{table*}[t]
  \setlength{\abovecaptionskip}{1pt}
   \setlength{\belowcaptionskip}{-0.0cm}
	\caption
	{
% 	\small	
		Fine-tuned image-text retrieval results on Flickr30K and COCO datasets.
	}
	\label{downmain}
    % \aboverulesep = 0.48mm
    % \belowrulesep = 0.48mm
    % \small
	\centering	
%  \setlength\tabcolsep{4pt}
%  \vspace{-3ex}
	\resizebox{0.83\textwidth}{!}
{
	\begin{tabular}	{l   |  c  c  c  c  c  c | c  c  c  c  c  c }
		\toprule	 	
	 \multirow{2}{*}{Method} & \multicolumn{6}{c|}{Flickr30K (1K test set)} & \multicolumn{6}{c}{MSCOCO (5K test set)} \\
	  &  \multicolumn{3}{c}{TR}& \multicolumn{3}{c|}{IR} &  \multicolumn{3}{c}{TR}& \multicolumn{3}{c}{IR}\\
	 \midrule
	& R@1 &R@5&R@10& R@1 &R@5&R@10& R@1 &R@5&R@10& R@1 &R@5&R@10\\
	Vanilla  & 90.8 & 98.6 &99.3 &79.4 &94.9 &97.2 &70.5 &89.9 &94.6 &53.5 &79.3 &87.2 \\
	FairVLP  &90.8 & 98.8 & 98.3 & 78.9 & 94.8 & 97.3 & 70.3 &90.3 & 94.9 & 53.6 & 79.3 & 87.1 \\
	\bottomrule
	\end{tabular}
	}
% 	\vspace{-0.8ex}
% 	\caption
% 	{
% 	\small	
% 		Fine-tuned image-text retrieval results on Flickr30K and COCO datasets.
% 	}
	\vspace{-0.7ex}


\end{table*}





==> tables/retrieval_zeroshot.tex <==
\begin{table}[t]

  \setlength{\abovecaptionskip}{1pt}
%   \setlength{\belowcaptionskip}{-0.5cm}
  \caption{Zero-shot image-text retrieval results on Flickr30K.}
  	\label{downzero}
  
%     \small
% 	\centering	
%     \aboverulesep = 0.46mm
%     \belowrulesep = 0.46mm
% \setlength\tabcolsep{5pt}
% 	\resizebox{0.75\textwidth}{!}
{
	\begin{tabular}	{l   |  c  c  c  c  c  c  }
		\toprule	 	
	 \multirow{2}{*}{Method} & \multicolumn{6}{c}{Flickr30K (1K test set)}\\
	  &  \multicolumn{3}{c}{TR}& \multicolumn{3}{c}{IR} \\
	 \midrule
	&  R@1 &R@5&R@10& R@1 &R@5&R@10 \\
	%ImageBERT~\cite{ImageBERT} & 2M &70.7 & 90.2 & 94.0 & 54.3 & 79.6 & 87.5 \\
	Vanilla  & 83.6 & 95.7 & 97.7 & 68.7 & 89.2 & 93.9 \\
	FairVLP  & 88.0 & 98.7 & 99.4 & 68.7 & 90.6 & 95.2 \\

		\bottomrule
	\end{tabular}
%  	}
%  	 \vspace{-0.8ex}
% 	\caption
% 	{
% % 	\small	
% 		
% 	}
}
    % \vspace{-0.7ex}
\end{table}		

==> tables/table4.tex <==
\begin{table}[t!]

\caption{\textbf{The results of multiple biases debiasing.} Bias$_m$ and Bias$_y$ respectively represent the \emph{male} bias and \emph{young} bias in mitigation of corresponding single bias. Fair Acc.$@$2, Bias$_m@$2 and Bias$_y@$2 denote accuracy, \emph{male} bias and \emph{young} bias, respectively, when both biases are eliminated simultaneously.} 
\vspace{-5pt}


\centering
\resizebox{0.47\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{Fair Acc.} & \multirow{2}{*}{Fair Acc.@2}& \multirow{2}{*}{Bias$_m$} & \multirow{2}{*}{\textbf{Bias$_m$@2}}& \multirow{2}{*}{Bias$_y$}& \multirow{2}{*}{\textbf{Bias$_y$@2}} \\
&&&&&&
\\
\cmidrule[0.5pt]{1-7} \morecmidrules\cmidrule[0.5pt]{1-7}
\textit{Vanilla} & 77.15 & 77.15 &26.24& 26.24 & 20.52& 20.52   \\ \midrule
\textit{AdvDebias} &\textcolor{blue}{77.62}  & \textcolor{red}{64.21} &11.56& 48.28 & 10.48 & \textbf{7.98}    \\ 
\textit{LNL} & 76.85 & 76.85 &26.43& 28.83 & 19.19 & 23.91   \\ 
\textit{EnD} & 77.11 & 76.83 &24.64& 24.95 & 21.57 & 25.88  \\
\textit{MFD} & 77.26 & 77.20 &20.17& 26.23 & 22.00 & 21.42  \\ 
\textit{DI} & 77.61 & 77.41 &23.01& 24.48 & 17.17& 17.59  \\  
\midrule
\textit{Active SD} & 78.63 & \textbf{77.84} &7.33& \textbf{3.73} & 14.31  & 14.57  \\ \bottomrule
\end{tabular}
}

\label{table:multibias}
\end{table}





